A Framework for Proof-carrying Logical Transformations

In various provers and deductive verification tools, logical transformations are used extensively in order to reduce a proof task into a number of simpler tasks. Logical transformations are often part of the trusted base of such tools. In this paper, we develop a framework to improve confidence in their results. We follow a modular and skeptical approach: transformations are instrumented independently of each other and produce certificates that are checked by a third-party tool. Logical transformations are considered in a higher-order logic, with type polymorphism and built-in theories such as equality and integer arithmetic. We develop a language of proof certificates for them and use it to implement the full chain of certificate generation and certificate verification.

==> eptcsdata.tex <==
\providecommand{\firstpage}{5}
\providecommand{\publicationstatus}{Chantal Keller and Mathias Fleury (Eds.): Seventh Workshop\\
on Proof eXchange for Theorem Proving (PxTP)\\
EPTCS 336, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.336.2}{10.4204/EPTCS.336.2}}
\pdfoutput=1

